Fast and Reliable Missing Data Contingency Analysis with Predicate-Constraints

Today, data analysts largely rely on intuition to determine whether missing or withheld rows of a dataset significantly affect their analyses. We propose a framework that can produce automatic contingency analysis, i.e., the range of values an aggregate SQL query could take, under formal constraints describing the variation and frequency of missing data tuples. We describe how to process SUM, COUNT, AVG, MIN, and MAX queries in these conditions resulting in hard error bounds with testable constraints. We propose an optimization algorithm based on an integer program that reconciles a set of such constraints, even if they are overlapping, conflicting, or unsatisfiable, into such bounds. Our experiments on real-world datasets against several statistical imputation and inference baselines show that statistical techniques can have a deceptively high error rate that is often unpredictable. In contrast, our framework offers hard bounds that are guaranteed to hold if the constraints are not violated. In spite of these hard bounds, we show competitive accuracy to statistical baselines.

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}

==> bak.tex <==

\subsection*{Application 1. Opportunistic Constraint Caching}\label{sec:application1}
An overarching question is from where does a user derive such constraints. We present three example application scenarios that are also reflected in our experiments.
Consider a large analytics database that is being used for exploratory data analysis.
Users issues aggregate queries to this database.
If the database is large-enough, these aggregate queries can take a significant amount of time.

We propose to \emph{opportunistically} (meaning as a consequence of execution) cache constraints on the data.
As aggregates are processed, we can calculate min and max values for the aggregated attribute within a predicate and its selectivity.
As time goes on, more and more of these predicate, min, max, selectivity tuples will be collected and will overlap in complex ways.
Our framework can allow a user to directly query this set of overlapping constraints to get an upper and lower bound on their query result (it is possible that their result is unbounded).

\comment{
Consider the following two queries:

Q1:
\begin{lstlisting}
SELECT COUNT(1)
FROM USA, CITY, YEAR
WHERE USA.city = CITY.city 
AND YEAR.year = USA.year
GROUP BY CITY.state
\end{lstlisting}

Q2:
\begin{lstlisting}
SELECT COUNT(1)
FROM USA, CITY, YEAR
WHERE USA.city = CITY.city 
AND YEAR.year = USA.year
AND USA.year = 2000
GROUP BY CITY.state, CITY.region
\end{lstlisting}

There are two approaches we can build constraints opportunistically, a \textbf{top-down} approach leverage the result of the previous query directly, e.g., in Q1, because of the group-by, we are able to collect a constraint for all value in the CITY.state domain, and the constraint is about the joined relation of the three tables. Since Q2 is querying a subset of data covered by constraint collected from Q1, we can produce an answer based on the constraints we collected. 

Naively, the approximate result for Q2 could be:

For each pair of $<state, region>$: 
    apply the constraint with the same state. 

But a concern of this approach is that the constraints we collect from different query might have totally different dimensions, for example, even though we can answer Q2 because predicates in Q2 is a subspace of the constraints we collect from Q1, the results will be very loose because there's no information about the YEAR in the constraint.

Informally, the algorithm can be described as below:

\textbf{Algorithm:} 

Input: 

\hspace*{6mm} $S$: a set of constraints collected opportunistically; 

\hspace*{6mm} $\mathcal{D}$: domain of each attribute;

\hspace*{6mm} $\pi_q$: a constraint generated from target query Q;

Step1: Find $S' \subset S$ that contains constraints relevant to Q. I.e. space represented by each constraint $\pi_i \in S'$ overlaps with $\pi_q$:

\[
    S' = \{\pi_i | \pi_i \cdot \pi_q \ne \mathbf{0}\}
\]

Step2: Check if $\pi_q$ can be bounded by $S'$, i.e. if $S'$ fully covers $\pi_q$. If not bounded, stop the algorithm.

Step3: We define $\pi_q$'s neighbor to be constraints that are overlapping with $\pi_q$ or $\pi_q$'s neighbor.  For pruning purpose, find a set of constraints $S''$ that are neighbors of $\pi_q$ then follow Section \ref{sec:cell-decomp} to perform cell decomposition, with an input Constraint set of $S'' \cup \pi_q$

Step4: Use ILP to find the optimal bound, subject to constraint of each cell and allocation to each cell is >= 0.

\textbf{Note}: Step2 is necessary because even if cells does not cover $\pi_q$ fully, ILP can still give a solution based on the constraint of cells ($\pi_q$ does not have a constraint, only predicates) but it is not a bound for $\pi_q$.

\textbf{Discussion}: As mentioned in Section \ref{sec:cell-decomp}, Step3 is $O(2^n)$ therefore very expensive to proceed. A simple group by queries would yields thousands of constraints that is too large to handle.

A sub-optimal goal would be to find a bound that is not optimal, one way is the following algorithm:


\textbf{A Sub-optimal Algorithm for a Loose Bound:}

Input: 

\hspace*{6mm} $S$: a set of constraints collected opportunistically; 

\hspace*{6mm} $\mathcal{D}$: domain of each attribute;

\hspace*{6mm} $\pi_q$: a constraint generated from target query Q;

Step1: Find $S' \subset S$ that contains constraints relevant to Q. I.e. space represented by each constraint $\pi_i \in S'$ overlaps with $\pi_q$:

\[
    S' = \{\pi_i | \pi_i \cdot \pi_q \ne \mathbf{0}\}
\]

Step2: Find a set of constraints $S_c$, $S_c \subset S'$ and each constraint $\pi_i \in S_c$ covers $\pi_q$, therefore, each of this specification can be used to bound Q. Let 

\[
    bound = Min(ExactBound(s, Q), s\in S_1).
\]

Step3: For $S_r = S' - S_c$, $S_r$ is the set of constraints that overlaps with $\pi_q$ but does not cover $\pi_q$. 

Step4: Group the constraints in $S_r$ by the dimension of their predicates, let $Sg$ be groups of constraints with the same dimension:


    for each group $Sg_i \in Sg$:
    
        \hspace*{6mm} if the union of constraints in $Sg_i$ covers Q:
        
        \hspace*{6mm} \hspace*{6mm} $bound = Min(ILPBound(Sg_i, Q), bound)$
        
        \hspace*{6mm} \hspace*{6mm} OR
        
        \hspace*{6mm} \hspace*{6mm} $bound = Min(ExactMatch(Sg_i, Q), bound)$

\textbf{Discussion}: In Step4, if the constraints in a group $Sg_i$ is still too large for cell decomposition, we can use ExactMatch to find a bound of $Sg_i$. A further optimization for this step is to find the optimal subset $Sg_i' \subset Sg_i$ that covers $\pi_q$. This can be modeled as a \textsf{Set Cover problem}: assume each $\pi_i \in Sg_i$ is of cost $c_i$ (can be cardinality or maxValue), the goal is to cover $\pi_q$ with $Sg_i' \subset Sg_i$ while minimize the cost of $Sg_i'$. It can be solved with ILP without cell decomposition and the result is fed to ExactMatch to generate a bound. However, the optimal bound is not guaranteed, it only generates a better sub-optimal bound.

A \textbf{bottom-up} approach leverage the fact that when we process the queries, we have to scan all the base tables. Therefore, we can build simple constraints for each base table and build up more complicated constraints by applying constraint operations as we process the sub-queries. This approach has less to do with the actual query result from previous query. With this approach, the quality of the result depends on how the base constraints are constructed, the attributes involved, the granularity of each constraint, etc. The disadvantage of this approach is that it might increase the overhead due to generating base constraint and manipulation of constraints. }

\subsection*{Application 2. Accounting For Missing Data}
Data completeness can becoming a significant roadblock for data analytics. Existing systems either pessimistically believe that missing information is completely gone or optimistically believe that missing information can be recovered by imputation.
Our framework can allow a user to strike a middle ground.
A user may have collected a dataset with an unknown number of tuples that are missing.
The user can define different contingencies on the values and the frequency of different tuples in the missing set.
Our framework can process queries over these contingencies to assess the worst-case impact of different scenarios.

\subsection*{Application 3. Data Cleaning}
Dirty numerical data is very challenging to curate. While there are several techniques for detecting outliers in numerical data~\citep{hellerstein2008quantitative}, recovering the true value is very challenging because there is an infinite range of true values that one could choose~\citep{chu2016data}. 
Our framework allows you to impute a range of values instead of a single value, and accordingly bound any subsequent query processing above and below.
Generally, such a ``range'' imputation is trivial-- either one processes the query with the high value or the low value in the range.
However, our general framework also allows one to specify global constraints that cross all the values.
For example, all values are within $0-100$ but no more than 10 are above $80$.

\subsection*{More Applications}
\begin{itemize}
    \item txn escrow
    \item differential privacy
    \item data skipping
\end{itemize}





The first constraint defines a global value constraint over all of the data:
\[ \pi_1 := true \implies (0 <= age <= 122)\]
This says that all records must have an \texttt{age} between 0 and 122.
The second constraint defines a conditional value constraint over the data:
\[ \pi_1 := \text{(pcp = 0332-4)} \implies (0 <= age <= 18)\]
This says that those records with the particular provider have an \texttt{age} between 0 and 18.
Finally, the last constraint defines a trivial value constraint but a frequency constraint over a predicate:
\[c3: \text{(100 <= age <=122)} \implies (100 <= age <=122)
\]
\[
freq((100 <= age <=122)) < 10
\]
This says that there can be no more than 10 tuples with an \texttt{age} greater than 100.
The predicate-constraint formalism allows us to express all of these different scenarios in one formal language.

\zs{removed the part of contradictory PC, and the following definition of covered PC. }
% However, arbitrary predicate-constraints can be contradictory. For example, one might have the constraint:
% \[(age >= 30) \implies (0 <= age <= 18)\]
% To avoid such situations, we restrict our study to non-contradictory predicate-constraints. But, simply ensuring that there exists a tuple that satisfies the constraint is not enough. We could have a situation like this:
% \[(age >= 10) \implies (0 <= age <= 18),\]
% where the predicate affects the possible value constraints.
% Intuitively, we need a notion of minimality, where the value constraints tightly bound the possible tuples that satisfy the constraints. In particular, minimality says that there exists at least 1 tuple that satisfies $\psi$ and each possible value contained in the value constraint.

% First, let us define some notation. Let $v$ be a possible value of attribute $a_i$, and let $\mathcal{D}_{a_i = v}$ be the set of tuples from the domain that have that value.

% \begin{definition}[Covered Attribute]
% Let $\pi = (\psi, \nu, \kappa)$ be a predicate-constraint, and for a value constraint on attribute $i$, let $\textsf{range}(l_i,h_i)$ denote a subset of an attribute's domain specified by the constraint. Attribute $i$ is covered if and only if for every value in the range there exists at least one tuple that satisfies $\psi$:
% \[
% \forall v \in \textsf{range}(l_i,h_i)~~~,~~~ \exists t \in \mathcal{D}_{a_i = v} : \psi(t)
% \]
% \end{definition}

% This leads to a natural definition of a covered predicate constraint. Where every value constraint is covered.

% \begin{definition}[Covered Predicate Constraint]
% Let $\pi = (\psi, \nu, \kappa)$ is covered if for every attribute $a_1,...a_i,...,a_p$ it's corresponding value constraint range $\textsf{range}(l_i,h_i)$ is covered.
% \end{definition}
\zs{removed the part of semiring of PC}

\comment{
        \subsection{Operations on Predicate-Constraints}
        We can define operations that manipulate predicate-constraints. 
        Let $\pi_i = (\psi_i,\nu_i, \kappa_i)$ and $\pi_j = (\psi_j,\nu_j, \kappa_j)$.
        The operation $\pi_i \cdot \pi_j$ is akin to an intersection of the two constraints:
        \[
        \pi_i \cdot \pi_j = (\psi_i \wedge \psi_j,\nu_i \cap \nu_j, \kappa_i \cap \kappa_j)
        \]
        There is further a multiplicative identity element, which does not constrain any tuples:
        \[
        \mathbf{1} = (true, \mathcal{D}, (0,\infty)) ~~,~~ \pi_i \cdot \mathbf{1} = \pi_i
        \]
        The intersection operation also gives us a natural definition of containment $\pi_i \subseteq \pi_j$ for predicate constraints:
        \[
        \pi_i \cdot \pi_j = \pi_i
        \]
        
        Likewise, the operation $\pi_i + \pi_j$ is akin to union of the two constraints:
        \[
        \pi_i + \pi_j = (\psi_i \vee \psi_j,\nu_i \cup \nu_j, \kappa_i \cup \kappa_j)
        \]
        Similar to multiplication, there is an additive identity element:
        \[
        \mathbf{0} = (false, \emptyset, (0,0)) ~~,~~ \pi_i + \mathbf{0} = \pi_i
        \]
        
        When we discuss bounding aggregate queries with joins and cartesian products it will be useful to consider a concatenation (direct-product) operator as well. Let $\pi_i$ and $\pi_j$ be two predicate constraints from two different relations. We assume the attributes are disjoint or labeled with the source relation (e.g., $R.a, T.a$). The direct-product operation is defined as:
        \[
        \pi_i \times \pi_j = (\psi_i \wedge \psi_j,[\nu_i \nu_j], \kappa_i \otimes \kappa_j)
        \]
        where we take a conjunction of the predicates, concatenate the value constraints, and take an element-wise product of the frequency constraints (multiply the lower bounds, and multiply the upper bounds).
        
        Finally, we also define the unary negation operation as:
        \[
        -\pi_i = (\neg \psi_i,\nu_i, \kappa_i)
        \]
        Additionally, there is a natural partial order over sets of predicate-constraints: \[\pi_i \preceq \pi_j  := \psi_i \implies \psi_j\]
        Intuitively, this means that every tuple that satisfies $\psi_i$ also satisfies $\psi_j$.
        
        \begin{proposition}
        The union $+$ and intersection $\cdot$ operations over predicate-constraints define a semiring.
        \end{proposition}
        
        \noindent \textbf{Remark: } While these semiring operations are exactly equivalent to their Boolean counterparts, as we will see later in the paper, the semiring notation (with $+$ and $\cdot$) will make certain definitions easier to express.
}

\zs{removed the part of consistency and closure}

\comment{
        \subsection{Predicate-Constraint Sets}
        A predicate-constraint set is defined as follows:
        \[
        \mathbf{S} = \{\pi_1,...,\pi_n\}
        \]
        The goal of this paper is to understand whether $\mathbf{S}$ gives us enough information to bound the results of common aggregate queries. We need to first describe regularity conditions on these predicate-constraint sets. For example,
        we could have a situation where two constraints:
        \[ \pi_1 := \text{(pcp = 0332-4)} \implies (0 <= age <= 18)\]
        \[ \pi_2 := \text{(pcp = 0332-4)} \implies (0 <= age <= 22)\]
        The challenge is that $\pi_1 \preceq \pi_2$ but $\pi_1 \not \subseteq \pi_2$.
        There is ambiguity on which constraint should be enforced.
        This leads to the definition of consistency:
        \begin{definition}[Consistency]
        Let $\mathcal{S}$ be a predicate-constraint set, and for any subset $S \subseteq \mathcal{S}$ let $\pi_S$ denote the union of all the constraints:
        \[
        \pi_S = \sum_{s \in S} \pi_s
        \]
        $\mathcal{S}$ is consistent if for any two subsets $S, T$:
        \[
        \pi_S \preceq \pi_{T} \implies \pi_S \subseteq \pi_T 
        \]
        \end{definition}
        
        The next regularity property is closure, which means that every tuple in the domain satisfies at least one of the predicates.
        \begin{definition}[Closure]
        Let $\mathbf{S}$ be a predicate constraint set with the elements $\pi_i = (\psi_i,\nu_i, \kappa_i)$
        $\mathbf{S}$ is closed over an attribute domain $\mathcal{D}$ if for every $t \in \mathcal{D}$:
        \[
        \exists \pi_i \in \mathbf{S}: \psi_i(t)
        \]
        \end{definition}
        Closure is akin to the traditional closed world assumption in logical systems, namely, the predicate constraints completely characterize the behavior of the relation over the domain. 
}

==> coverletter.tex <==
\begin{center}
\textbf{Cover Letter}    
\end{center}

We thank the reviewers for their careful review of our submission and have addressed every point laid out in the reviews. First, we summarize our problem setting below and the key result below:

\vspace{0.5em} \noindent \emph{Problem Setting. We are given a set of tables with an unknown number of missing rows. The user provides us with a set of constraints (called predicate constraints) that constrain the values and the number of these missing rows for each table. For an aggregation query, our framework returns a range of results consistent with those constraints. Crucially, we ensure the property that if the constraints are not violated the result is guaranteed to fall into the range.}

\vspace{0.5em} Below are the detailed changes in response to the issues raised by each reviewer. We have highlighted revisions to the text requested by reviewer 1 using a red text color, reviewer 2 using blue, reviewer 3 using green, and for multiple reviewers/changes not explicitly requested by the reviewers with purple. 


\vspace{.5cm}
\noindent{\textbf{Reviewer \#1}}

\Rev{R1.D2}{I think the ratio of missing rows could impact the quality of different methods. I could not find relevant information in the experiment setup section though. If the ratio indeed impacts the quality of different methods, it would be valuable to study it. If the ratio doesn’t impact the qualities, it would be nice to briefly describe this irrelevance.}

%done
\Ans{Added. We added clarifications that make the ratio of missing rows explicit and explain how that ratio affects accuracy in Section \ref{sec:missing_ratio}.}

\Rev{R1.D3}{It is great that the proposed approach ensures the correctness of bound. On the other hand, though, I’m curious how tight those bounds really were. Of course, giving bounds (-inf, inf) will always make the bounds correct although those bounds are quite useless. In this regard, I think it is also important to study the optimality of the bounds.}

%done
\Ans{Fixed. We apologize for the lack of clarity. All of our experiments evaluate tightness as well as correctness. Section~\ref{exp-setup} is revised to clarify our measure of tightness (the ratio of the confidence interval upper bound with the true result), and Section \ref{sec:missing_ratio}/\ref{exp-other} illustrates that PCs are competitively accurate with other baselines.}

\Rev{R1.D4}{ Considering the presidential election example, I think the final estimation should be a combination of sampling effect and missing rows. Specifically, a survey agent may choose 10,000 people for asking their opinions, some of which may not respond or falsely respond. Then, these numbers would have to be post-processed appropriately to estimate confidence intervals. I wonder if the proposed approach can be easily applied in this scenario.
}

%done
\Ans{This is a very insightful suggestion. The strength of statistical sampling is its ability to accurately estimate ``central'' values from complex distributions, e.g., mean, median, quartiles. However, sampling's key weakness is its ability to capture rare, extremal values such as the maximum value of a population. However, these rare values are exactly what trigger estimation failures. We believe that the two approaches can be brought together in a very powerful Approximate Query Processing system where sampling is used to produce approximate results and PCs generated from the data are used to produce confidence intervals.}

\Rev{R1 Required Changes for a Revision}{
R1 Please study the optimality of the bounds. (D3) I think it would be interesting to compare this against 99\% CLT and 99.9\% CLT in terms of both optimality and error ratios. *Clarification*: By "optimality", I think I meant the empirical accuracy or tightness of the computed bounds since if the proposed approach is designed to absolutely guarantee the correctness of those bounds, their sizes could be larger than statistical error bounds obtained from other sampling-based approaches (expectedly).}

%done
\Ans{
Added. Results on the accuracy and failure rate of sampling baseline and PC can be found in Section \ref{sec:fr-tradeoff}/\ref{sec:missing_ratio}/\ref{exp-other} of the paper. Beyond the reviewer's query, we expanded the evaluation to include 1000 random queries and return the median accuracy over these queries. Results suggest that despite the hard bounds, our framework is competitively accurate with sampling (even when the samples consider 10x more data!). Counter-intuitively, it is not always the case that sampling is more accurate. For highly selective predicates, a PC might capture key correlation information that results in a better estimate.
}

\newpage
\noindent{\textbf{Reviewer \#2} }

\Rev{R2.D1}{The main argument behind predicate constraints given in the paper is that they can accurately and deterministically give an upper bound on an aggregate function without requiring any assumption on distributions. On the other hand, in all the applications mentioned in the paper, it seems the predicate constraints are likely to be beliefs on the missing partitions, e.g., in 2.1, "From historical experience, the data scientist might guess that: between 10-20\% of the rows are from the age 18-25 age group and voted for ‘John Doe’, or 5-10\% of the rows in the same age group vote for the ‘Jane Smith’". Therefore, it seems that getting the upper bounds on the aggregates using predicate constraints can still be uncertain, while it misses the opportunity to use confidence intervals of statistical and probabilistic approaches}


%done
\Ans{We agree with this comment. PCs return a result range with a simple guarantee: if the rules described in the PCs are not violated, the true result is guaranteed to be inside the computed range. To the best of our knowledge, a comprehensive framework in the database literature that provides such a guarantee does not exist. If the PCs themselves are inaccurate or are guesses, then this guarantee is vacuous, of course. 

However, it is important to note the user could just as easily run into the same issue with a probabilistic technique as well. If a user mis-specifies her belief in the data distribution or sampling process, any inference would be equally fallible. Here are ways in which it could happen in the missing data setting:

\begin{enumerate}
    \item The user specifies a column with missing values is normally distributed when it is, in fact, distributed as a power law.
    \item The user specifies that two columns are independent when they are actually correlated through a third variable.
    \item The user specifies that the data are missing at random when in fact there is a temporal correlation to the missing data.
\end{enumerate}

We argue that retroactively testing for a mis-specified PC is far easier to do than it is for probabilistic specifications. PCs are similar to integrity constraints and can be evaluated with SQL queries on historical or held-out data. Testing a probabilistic property like conditional dependence could be very challenging, if not intractable, for complex dependence relationships. 

Despite this simplification, our experiments show competitive accuracy with more general sampling/probabilistic techniques. We also believe that the ideas presented in the paper are complementary to probabilistic inference. See our response to R1.D4. }


\Rev{R2.D2}{It would be good to add an example for Def 3.2 closure - e.g., when the age distribution for all the tuples are given?}

%done
\Ans{Added. Section~\ref{closure} includes an example using age distributions.}

\Rev{R2.D3}{The NP-hardness proof in Proposition \ref{proposition41} is about combined complexity (both data and queries/constraints are variable), whereas in practice, I assume the number of constraints will be small. It would be interesting to know whether the problem is also hard in terms of data complexity.}

%done
\Ans{We apologize for a confusing discussion about this point in the Author Response period, partially because the query made by the reviewer is very subtle and required a longer reflection. Part of the confusion arises from the fact that query and data complexity have specific definitions in database theory, and those definitions are not exactly relevant in our setting. We find the results are not particularly informative. Thus, we will exclude this discussion from the paper (unless the reviewers request us to add it).

First, we can define a restricted version of the problem addressed in the paper: 
\begin{definition}[Predicate-Constraint Optimization Problem]
Let $\pi_i$ be a predicate-constraint whose predicate is expressed in Disjunctive Normal Form with at most $k$ equality clauses on a single attribute (attribute equal to a constant). Let $P$ be a set of $n$ predicate-constraints. The predicate-constraint optimization problem is to find the maximal sum possible if a single table were to satisfy all $n$ predicate constraints.
\end{definition}

Based on this definition, we can appropriately define data and query complexity:
\begin{definition}[Data Complexity]
The data complexity of the predicate-constraint optimization problem is the number of computational steps required to solve the optimization problem for a fixed $k$ and a variable $n$.
\end{definition}

To summarize the key results below (if requested we can include these in the paper), 
\begin{itemize}
    \item For $k\le 1$, the data complexity is $\mathcal{O}(n)$. In this setting, there are only two possibilities: either two PCs fully overlap or they are disjoint. The complexity of the problem arises because we have to reason about interactions between the predicates.
    \item For $k\ge 2$, the problem is NP-Hard by reduction to a maximal independent set problem: there exists a predicate-constraint optimization problem instance for $k=2$ that is NP-Complete.
    \item For $k\ge 2$, in the special case, where each PC's predicate is disjoint from all other predicates, the data complexity is $\mathcal{O}(n)$.
\end{itemize}

\begin{definition}[Query Complexity]
The query complexity of the predicate-constraint optimization problem is the number of computational steps required to solve the optimization problem for a fixed $n$ and a variable $k$.
\end{definition}

The complexity of the query plays a role in determining the set of disjoint cells. For the restricted problem above, e.g., disjoint, the query complexity is actually linear in $k$ (for predicates that are a disjunction of equality statements). To calculate overlaps between PCs, one simply looks for exact collisions over any of the clauses. \emph{However, we argue that this result is uninformative because the constant factor due to $n$ can be very large and is highly problem dependent. When the PCs are disjoint, this constant factor is $O(n)$, but in the worst case, it can be $O(2^n)$.} Also, this discussion on complexity only considers the worst-case running time and not the accuracy. Therefore, we believe it is most informative to look at the combined complexity setting as presented in the paper, which gives the user general intuition about why the problem is hard in the absolute worst case and experimental results about the practical accuracy.}

\Rev{R2.D4}{I am not sure if I am missing it but I cannot find the number of tuples in the datasets used, which is critical to understand the efficiency of the approach and its effectiveness.
I also do not see if the fraction of missing data has been varied in one of the experiments.}

%done
\Ans{We clarified the number of rows of each dataset in Section \ref{sec:missing_ratio} and \ref{exp-other}. Section \ref{sec:missing_ratio} presents the accuracy of our framework and baselines for different numbers of missing rows.}

\Rev{R2.D5}{The sampling techniques should be discussed before experiments.}

%done
\Ans{Fixed. The sampling techniques and our experimental notation are described in \ref{sampling}.}

\Rev{R2.D6}{Overall, I think the paper has good technical contributions for the in-depth study of predicate constraints, with analysis, optimizations, and detailed experimental evaluation (except that I am not sure of the number of tuples used in the experiments). The results are not completely surprising, but give a good overview of the problem. My main concern is the applicability of this approach in practice. Unfortunately I am not too excited about this paper in its current form.} 

%done
\Ans{Here are three real-world scenarios in which you will require a framework like the one described in this paper. We have modified Section 2 accordingly to describe these applications: 

\begin{itemize}
    \item A user wants to query a partitioned or federated dataset where there is some cost to reading an entire partition. Each partition, can be annotated with PCs to give users a sense of what the partition contains and how that might impact her results. Our framework can compute a range of possible values for a given query result without reading the data and requires substantially fewer data to do so than a statistical sampling method.
    \item Suppose that due to a server-outage a website’s access log data is lost for a few hours. A data scientist needs to write a report on the aggregate website’s traffic despite this data loss. The PC framework allows her to formally specify what she is assuming about the missing data (in terms of PCs), and return range of values that satisfy those assumptions. The practical side of the PC framework allows for those ``assumptions'' to be stored and versions just like code.
    \item Many approximate query processing (AQP) systems use samples to estimate query results and return confidence intervals that quantify how uncertain the results are. As seen in our paper, sampling is a poor measure of extremal values (minima and maxima) and rare events. The PC framework can augment existing AQP systems with bolt-on deterministic confidence intervals based on a small amount of meta-data.
\end{itemize}
}


\Rev{R2 Required Changes for a Revision}{
I am not fully convinced with the authors' response , but I am willing to see whether these concerns are addressed satisfactorily in a revision.

For instance:
R2D3: Like AQP, our algorithm has a constant data complexity."

I do not understand either part of the comment -- AQP has constant data complexity or the algo in the paper has constant data complexity -- this would mean that both of these would look at only a fixed number of tuples (5, 10, .. or a number that depends only on the schema like the no. of relations or attributes). Similarly I did not follow the response for R2D1 . I would appreciate if the changes are highlighted by a different color.
}
%done
\Ans{See above. We misunderstood the reviewer query during the author response, and have clarified accordingly.}

\vspace{0.5cm}
\noindent{\textbf{Reviewer \#3}}

%done
\Rev{R3.D1}{D1. Section 1: " If the query is unboundable given the constraints, the algorithm returns a failure." But notice that statistical may still be able to give you some bound. Thus this is an example where statistical methods can clearly give better bounds}

\Ans{Fixed. We have revised this discussion accordingly, and it was an unnecessary technicality on our part to introduce so early in the paper. In our framework, the set of PCs completely determines all assumptions made about the missing data. An ``unbounded answer'' could happen is if a user was aggregating an attribute without any constraints specified. In this case, the solving algorithm would predictably return an infinite value. It is worth noting that in a probabilistic framework, mis-specified or incorrect assumptions (see R2.D1 response above), can lead to undetected systematic errors in estimation---at least an infinite value indicates the problem is under-determined. }


\Rev{R3.D2}{The paper would benefit by bringing early an intuitive example that shows step-by-step the framework applied to example made-up data. Currently, as the paper is written, the first few pages discuss the problem at a very high-level. Then when the framework is introduced, there are obvious inconsistencies, which make it extremely unpleasant for a reader to have to guess in what ways the previous descriptions to actually interpret. For example, section 2.1 "Applications": "… Normally, this metadata is used for data skipping [30] but it is exactly in constraint format expected by our framework -- a predicate, a range, and a size." At that point predicate, range and size are not yet defined.}

\Ans{Major Change. We reorganized the paper and revised the example in Section \ref{sec:ex-application}. We also have added a toy numerical example in Section \ref{quant-ex} that explains how the optimization works.}

\Rev{R3.D2.2}{ section 2.1 Application 1: It is not obvious that running this modified algorithm is significantly less expensive than sampling the entire dataset. In the end, it is not entirely clear what the running time exactly depends on. Is it just the number of PCs? Does it depend on k?}
\Ans{In retrospect, this example is confusing and we have removed it from the paper.}


\Rev{R3.D3}{Section 2.2. There are n tables and n constraints. Does this imply one constraint per relation? I assume not and rather that care was not taken in the assignment of variables. Section 6.1 later uses "N" instead of "n" for number of PCs}

\Ans{Fixed. Each relation can have an arbitrary number of PCs. We have fixed the notation in the revision.}

\Rev{R3.D4}{ Section 2.2.: "Predicate Constraints are a sparse generalization of histograms. A histogram can be considered a 1-D dense predicate constraint which defines a partition of an attribute (a predicate) and the fraction of rows in that partition. Instead of a partition of a single attribute, a predicate constraint defines a general logical predicate and the attribute ranges of rows contained in that predicate." That discussion is very hard to follow without yet having seen any real example of a "Predicate Constraint". I had to give up parsing this sentence after a few times.
}

\Rev{R3.D5}{Similar with this later sentence: " Result ranges derived from predicate-constraints only fail if the constraints themselves are violated (or specified incorrectly) there are no random failures." Hard to swallow before ever seeing a "Predicate Constraint"
}

\Ans{Fixed. We reorganized the paper to avoid such confusion, and ensure a formal introduction of PCs can be found in Section \ref{sec:pc}.}


\Rev{R3.D6}{
 Section 3.1: Predicate: "For efficient implementation, we focus on predicates that are conjunctions of ranges and inequalities. " At a point when the whole formalisms is not yet introduced (which later turns out to be NP-complete), there is already a restriction of the language for efficiency reasons. It would have been helpful to explain why this restriction is necessary, at least later. Or a discussion on why this restriction is reasonable and still gives a framework useful in practice.
}
\Ans{Fixed. We reorganized the paper and include a forward reference to Section \ref{sec:cell-decomp} where the restriction is actually used.}

\Rev{R3.D7}{
The main definition and example of Predicate Constraint appears to be flawed. In multiple ways.
First, contrast:
1. a predicate appear to hold on the row, and a frequency constraint that "bounds the number of times that rows with the predicate appear." Later: "For all rows that satisfy the predicate, the values are bounded by and the number of such rows is bounded by"
2. Suppose, the data analyst wants to see what would happen if there are between 2 and 5 people in the age range who vote for `John Doe' and 13 people in that range that vote for `Jane Smith' :

Then definition 1. and example 2. are contradictory. According to the definition, c1 stats that there are between 2 and 5 rows that have the predicate "($18 \le age \le 25$)", not the predicate "($18 \le age\le 25$) and voting for 'John Doe'"

Also notice the definition of the cardinality constraint does not make logical sense:

Clearly the universal quantification needs to be removed.

For author feedback: please correct me in case I messed something up when reading the example above or the definition.
}

\Ans{ 
Fixed. We apologize for a handful LATEX issues that made the formulas difficult to read. Please see the revised version of Section \ref{sec:pc}.
}

\Rev{R3.D8}{
 Section 3.3: it would have been helpful to have a more detailed discussion on what c-tables can that PC cannot and v.v. This paragraph is hard to follow without an simple illustrating example. Same with m-tables
Also “we can express a limited number of open-world models”: What does this exactly mean?
}
\Ans{Fixed. m-tables do not provide an algorithm for bounding the effects of missing rows in aggregate queries, which is a core contribution of our work. We now discuss c-tables and m-tables further in Section \ref{sec:related}.}

\Rev{R3.D9}{
Section 4.1 "First, there is a potentially exponential number of cells." How come? Exponential in what? Number of PCs? In case that is so, then those are not that many, right?
}

\Ans{Here are clarifications that we have added to the paper:
\begin{enumerate}
    \item In the un-optimized algorithm, the number of cells is exponential in the number of PCs in the worst case. While generally the number of PCs is small, this growth is significant enough to warrant optimization techniques to avoid solving a MILP with that number of constraints.
    \item In the optimized algorithm (using the techniques described in Section \ref{sec:cell-decomp}), the number of cells is exponential to the \emph{number of PCS that overlap with the aggregate query predicate}.
    \item Results suggest a nearly 100x speedup with the optimizations \ref{exp-scaling}.
\end{enumerate}
}

\Rev{R3.D10}{
Optimization 3. How is this related to resolution?
}

\Ans{Optimization 3 is a special case of resolution that shows up extensively in our cell-decomposition problem. }

\Rev{R3.D10.2}{
Section 4.2: The output of the program seems to be how many rows are allocated to each range (X). Don't we also need the corresponding $U_i$? Also, I don’t understand how the approaches uses this to compute aggregates other than max. For example, COUNT says we set $X_i=1 $ but $X_i$ is the variable of the program, how will we “set it” to 1?
}

\Ans{Fixed. This is a typo, $X_i$ should be $U_i$. We fixed it in the revision.
}


\Rev{R3.D11}{
Section 5.2: "without loss of generality we assume attribute comes from the relation." But can't an attribute come from more than one relation?
}

\Ans{Fixed. We have added a note to this effect. We can very easily handle such queries but chose to exclude them from the discussion because they have an esoteric form of aggregation on a join key.}


\Rev{D3.D11.1}{
Also, this approach seems to work only for SUM. How do we do the other aggregates?
}

\Ans{Fixed. We have added clearer details for other queries can be found in Section \ref{sec:ilp}, all experiments include SUM and COUNT queries, and Section 6.9 shows results for all other types of queries.}

\Rev{D3.D12}{
D12. Section 7: "Especially for selective queries, these estimates can be highly fallible 95\% confidence interval may fail significantly more than 5\% of the time [1]. Unfortunately, as confidence intervals become more conservative, e.g., using more general statistical bounding techniques, their utility drops."
The experiments appear to use 99\% confidence bounds. Why the difference?
A key issue I a missing with this paper is more intuition: how is it possible that statistical methods (which allow some errors) would give worse or equal bounds, then a deterministic approach that by definition gives a 100\% confidence interval? That cannot hold universally. There needs to be some trade-off. And this trade-off is not clear. Partially because the paper unfortunately misses such a detailed discussion (why or when would this deterministic method work, when would it work worse, and why are the former cases where it works better common enough to care?). Also, because the paper misses in my opinion enough intuitive example that help a reader at least estimate for themselves the pluses and the minuses (or the hidden assumptions) to understand that trade-off themselves.
}

\Ans{Major change. We apologize for the lack of clarity and have significantly restructured the experiment section to illustrate these points, which are all valid.

\begin{enumerate}
    \item Figure \ref{se-teaser} in the background section shows why we can't simply use extrapolation to deal with missing rows. It shows that accuracy suffers when those rows are correlated with the aggregation.
    \item Section \ref{sec:missing_ratio} compares the PC framework against a $99.99\%$ confidence interval in a more clear way. PCs are more accurate than a sampling baseline when the dataset is subdivided (with the ``predicates'') in a way that is correlated with the aggregation of interest, random PCs are less accurate. However, both schemes have a 0\% failure rate.
    \item Section \ref{sec:fr-tradeoff} shows that by manipulating the confidence level (e.g., $95\%$ or $80\%$) , there isn't a good way to tune a sampling approach to avoid this pitfall. Small samples are simply a poor measure of extremal values (minima and maxima), and the presence of these values is a key reason for the result to fall outside the confidence intervals.
    \item The only real way to ``fix'' this issue with sampling is to massively expand the sample size (Section \ref{exp-data}). When the sample size is 10x the number of PCs, then sampling is more accurate at a 99.99\% confidence interval.
\end{enumerate}

These results should not be surprising. PCs are user-given information about the extreme values of missing data. Naturally, they are very efficient ``sketches'' of the range of values queries can take. One would choose to use sampling in a setting where an accurate generation of PCs was not possible or grossly inefficient compared to generating independent random observations of data. 
}

\Rev{R3.D13}{
D13: Section 6.7: Where exactly is the noise added? The range of the predicates?
}
\Ans{Fixed. Section \ref{exp-robustness} now explains that we add independent random noise to the attribute ranges of the predicate}

\Rev{Request for a Revision}{
Comments after reading the author's response:

The authors promise to fix the various errors, typos, omissions and unintuitive formalism, and add early intuitive and fixed examples (see list D1-D13 above). I now also support a revision and look forward to the updated revision.

More comments on the responses:

D14:
"R2D3: Like AQP, our algorithm has a constant data complexity." 

AQP has constant data complexity??? Please elaborate

D15:
"R3D1: Sampling methods are effective when the sampling process is fully under the control of the user, but less so when extrapolating the effects of naturally missing data correlated with values. While sampling can produce a result, there is often no guidance on whether that result is meaningful or not."

Please elaborate on the assumptions of this framework. In particular the assumption of available additional information. And the trade-off when this approach shines, and when it will not. Thus the reader would appreciate an honest discussion of pros and cons.

D16:
"1. There is no such thing as a 100\% statistical confidence interval, because with most statistical approaches there is always some probability that the world will give you a pathological sample (-inf, inf)."
 
But statistical approaches have the option to choose 95\% confidence and still return something that is "not too much" off on average. Again, please elaborate on this in the pros and cons
}

\Ans{D14: Please refer to R2.D3 for a detailed discussion on complexity. We apologize for a confusing response to the initial review, partially because the question is a little more subtle than could be adequately answered in the span of a week. If the reviewers find this discussion interesting we would be happy to include it in the paper.}

\Ans{D15. PCs are logical constraints that describe a user's belief in the number and distribution of missing rows. Two other ways to construct a ``belief'' would be to provide a small subset of missing rows (sampling) or provide a probabilistic model (a GMM in our experiments). For the same amount of data provided, we compare the accuracy of all the approaches. Here are the basic considerations:
\begin{enumerate}
    \item PCs produce deterministic bounds that are guaranteed to hold if the PCs are accurate. 
    \item The bounds themselves are just as ``tight'' as those from probabilistic methods \emph{if the PCs are generated on predicates that are meaningfully correlated with the aggregates of interest.}
    \item It takes roughly a $10n$-sized uniform random sample to match the accuracy of $n$ PCs when those PCs are appropriately correlated with the aggregate.
\end{enumerate}
The conclusion is that if one has a way of constructing accurate PCs, e.g., based on the expected workload, it is a far more data efficient sketch than a random sample with the added benefit of deterministic confidence intervals. The reasons for this are now described in Section \ref{sec:fr-tradeoff}.}

\Ans{D16. Fixed. Section \ref{sec:fr-tradeoff} shows the tradeoff in detail.}

==> extra-experiments.tex <==

\subsubsection{Election Campaign Expense Dataset}

The election campaign expenditure dataset \footnote{https://classic.fec.gov/disclosurep/PDownload.do} contains all campaign expense between July 2016 and September 2019 for the 2020 US Presidential Election. The dataset contains 71688 rows and 17 columns like candidate name, recipient name, disbursement amount, disbursement date, etc. 

We use this dataset to demonstrate the first scenario of using our framework in which a set of predicate-constraints of the whole dataset is available (e.g. pre-generated by a program). We term such a set of constraints `a \textbf{partition} of the dataset' because each constraint describes a part of the dataset and the whole dataset is covered by their union. Also, to simplify computation and to provide more accurate information, constraints could be designed to have other traits, e.g., of the same dimension, be disjoint to each other, etc. We can use such partitions to efficiently estimate the results of SPJA queries.

There are different ways to generate partitions, for example we could generate several orthogonal partitions, each partition split the dataset on a different dimension (attribute). The set of orthogonal partitions is then used as input to our framework. In this case a constraint from a partition only contains one predicate on the dimension that is used by the partition. 

We could also generate a partition by merging different dimensions into one constraint, for example, by using 2 dimensions, in each constraint, we can generate a `rectangle-shaped' predicates that contain predicates from 2 dimensions. Assume we want to generate a set of predicate constraints using $N$ dimensions, and each dimension is split into $K$ chunks, the size of the set of constaints will be $K^N$.

With a pre-generated `rectangle-shaped` partition of the dataset, we use our Predicate-Constraint framework to estimate queries of the following templates. 

\begin{lstlisting}
SELECT COUNT(*) FROM expense
WHERE pred1 AND pred2 AND ...
\end{lstlisting}

\begin{lstlisting}
SELECT SUM(disbursement_amt) 
FROM expense
WHERE pred1 AND pred2 AND ...
\end{lstlisting}

For each query template, we generate 100 test queries with random predicates, we apply our framework to estimate the query result and evaluate the result with 2 metrics: 1) the correctness, i.e. whether the result is a bound to the actual query result and 2) the optimality of the bound, i.e. how close the result to the ground truth. We compare our approach with a 10$\%$-sample AQP.

Unsurprisingly, even though AQP produces a result that is relatively close to the ground truth, it is not reliable. For the 100 COUNT queries, AQP successfully bounds 74 of them which yields a success rate of 74$\%$. However, AQP only bounds 7 of the 100 SUM queries thus yields a success rate of 7$\%$. On the other hand, our framework always generates a bound.

To apply the Predicate Constraint framework, we generate a partitions of the dataset using two dimensions (file$\_$number and disbursement$\_$date) and varies how many chunks to split each dimension into. As we increases the number of chunks in each dimension, the predicate constraints will become more fine-grain thus be able to provide more accurate information.

Figure \ref{fec-count} shows the results for the 100 random COUNT queries, we compare the average ground truth with the average bound derived with our framework using different type of partition, e.g. 10x10 means each dimension is split into 10 chunks. We can see as we increase the quality of the partition, the gap between the bound and ground truth shrinks. In fact, if we treat each tuple in the dataset as a partition, our framework will generate a bound that matches the ground truth. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.88\linewidth]{exp-figures/fec-count.png}
    \caption{We compare the average bound of 100 random COUNT queries derived by Predicate Constraint using different partition with the average of ground truth.}
    \label{fec-count}
\end{figure}

For the SUM queries, the gap between the bound and ground truth increases significantly because of the skew of the aggregated attribute: to make sure we always bound the worst case, our approach assumes that all tuples in the same predicate constraint share the maximum value of the aggregated attribute. We believe the bound will be tighter for attributes whose values are more evenly distributed.

Therefore, in Figure \ref{fec-sum},  instead of showing the absolute value, we show the average difference in the magnitude of the bound and the ground truth. We can see that as we increases the quality of the partition, the bound can be less than 2-magnitude of the ground truth. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.88\linewidth]{exp-figures/fec-sum.png}
    \caption{We compare the bound of 100 random SUM queries derived by Predicate Constraint using different partition with the ground truth, due to the skew of the aggregated attribute, we show the average difference in magnitude of the two values.}
    \label{fec-sum}
\end{figure}


\subsubsection{Intel Wireless Dateset}

\textbf{Texts to be updated for figures}
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{exp-figures/intel-deviceid-time.pdf}
    \caption{Baseline performance on 100 COUNT(*) and SUM queries with predicate attributes on \textit{DeviceId} and \textit{Time}.}
    \label{intel-id-time}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{exp-figures/intel-deviceid.pdf}
    \caption{Baseline performance on 100 COUNT(*) and SUM queries with predicate attributes on \textit{DeviceId}.}
    \label{intel-id}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{exp-figures/intel-time.pdf}
    \caption{Baseline performance on 100 COUNT(*) and SUM queries with predicate attributes on \textit{Time}.}
    \label{intel-time}
\end{figure}

The Intel wireless dataset \cite{intelwireless} contains data collected from 54 sensors deployed in the Intel Berkeley Research lab in 2004. This dataset contains 8 columns including different measurements like humidity, temperature, light, voltage as well as date and time of each record.

We use this dataset to demonstrate how to use our framework to handle a `missing data` situation. In the missing data problem setting, we assume partial of the dataset is missing and a nice partition of the dataset is not available. Instead, we have a predicate constraint set that might not be well-formed (e.g. inferred from a survey or recalled from a vague memory of the DBA, etc). The set of constraints could be arbitrarily organized (e.g. overlaps in a tricky way so that a greedy algorithm fails). We want to estimate the maximum impact of the missing data described by the predicate constraint set to the query result.

We focus on constraint that contains the date and epoch column (can be easily extended to more dimensions) and randomly generated 100 test cases, each test case contains a set of 20 constraints, i.e. data described by this 20 constraints are missing. 

For each test case, we are interested in estimating the impact of the missing data to the following queries:

\begin{lstlisting}
SELECT COUNT(1) FROM data;
SELECT SUM(Voltage) FROM data;
SELECT SUM(Light) FROM data;
\end{lstlisting}

We also compare our solving technique with different baselines: 1) ExactBound, a naive heuristic based baseline that always assumes the constraints are disjoint therefore simply sum up all the constraints to derive a bound, 2) SampleBound, a sampling approach that tries to assign tuples randomly to each predicates until it finds an allocation that does not violate any constraint, and 3) Greedy, a greedy algorithm that prefers to satisfy allocations with fewer constraints first. For each of the baseline, we also evaluate their success rate and their optimality.

Figure \ref{intel-count1}, \ref{intel-sumv} and \ref{intel-suml} shows the results on the COUNT(1) query, SUM(Voltage) and SUM(Light) query respectively. We can see that the heuristic-based baselines works well on the COUNT(1) query but are very loose. Due to its heuristic of counting every possible tuple without considering constraint, the ExactBound always over-estimate thus produce very loose bound. We also notice that the Greedy baseline works the same as the Linear Programing baseline, always produce the optimal result that can bound the worst case, this is because the test cases we generated are not complicate enough to distinguish the two. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\linewidth]{exp-figures/count1-fr.png}
    \includegraphics[width=0.48\linewidth]{exp-figures/count1-dist.png}
    \caption{Baseline performance on the COUNT(1) query.}
    \label{intel-count1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\linewidth]{exp-figures/sumv-fr.png}
    \includegraphics[width=0.48\linewidth]{exp-figures/sumv-dist.png}
    \caption{Baseline performance on the SUM(voltage) query}
    \label{intel-sumv}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\linewidth]{exp-figures/suml-fr.png}
    \includegraphics[width=0.48\linewidth]{exp-figures/suml-dist.png}
    \caption{Baseline performance on the SUM(light) query}
    \label{intel-suml}
\end{figure}

As expected, the failure rate of the sampling-based baselines decreases as the number of sampling increases. A surprising yet reasonable observation is that the sampling-based baselines with a higher than 40\% failure rate on the COUNT(1) query outperform the Linear Programming baseline on the SUM(LIGHT) query. This is reasonable because the $Light$ attribute has a large standard deviation which means there is a large gap between its mean and max value. As a result, for the SUM(Light) query, even though the sampling-based baselines failed to bound the COUNT(1) query, the summation of the multiplication between the underestimated allocation (i.e. how many tuples are assigned to a specification) and the overestimated value (i.e. the max value) of the missing tuples exceed the true value. Therefore, we can conclude that the performance of the baselines on the value aggregate functions like MIN, MAX, AVG and SUM also depend on the value of the aggregated attribute.


\subsubsection{Census Dateset}

In this experiment, we showcase the third scenario of using predicate-constraint where we collect constraints in a opportunistic manner, i.e. every time a query is processed, we bookkeep the predicate used by the query and the result of the predicate and use it to form new constraints that can be used to process future queries. 

We use CUBELOAD\cite{rizzi2014cubeload} to generate a workload of 100 queries. CUBELOAD simulates real-life usage of OLAP systems by generating workloads that contain multiple query sessions, each session is generated by using one of its 4 templates of different characteristics, e.g. in a Slice-and-Drill session, user might start by querying a sales report per state and year, then dig into a particular year or a particular state in later queries. 

The dataset that is used by CUBELOAD is IPUMS\cite{steven2019ipums}, which contains census data from 2015, as described earlier, the IPUMS dataset contains a fact table and several dimenstion tables. Each tuple in the fact table describe a different aspect of the census, e.g. the occupation, race, residency of an individual. And the dimension tables like OCCUPATION, RACE, CITY can be joined with the fact table to provide verbose information of the census. Queries generated by CUBELOAD are of the following form:

\begin{lstlisting}
SELECT COUNT(1)
FROM Table1, Table2, ...
WHERE Predicate1 AND Predicate2, ... 
GROUP BY Column1, Column2, ...
\end{lstlisting}

To handle the group-bys, we decompose the group-bys to predicates using the domain of the group-by columns, therefore each query with a group-by condition is substituted with one or more queries. 

The queries are processed in a first arrive first serve manner. Every time the execution engine processed a query, we opportunistically collect a constraint by tracking the predicates of the query and the cardinality of the query result. Note that constraint caching could also be more aggressive by leveraging the intermittent query results from the optimizer but in this experiment we only cache one constraint based on the entire query. The collection of constraints will keep growing as we execute more queries (currently we do not enforce a storage constraint), and the previously collected constraints are used to evaluate the upcoming queries. We record the result generated by using predicate-constraints and compare to a simple AQP baseline in which we execute the query with 20\% of the data.

For each query, we first solve it with the constraints we have collected and record the bound that is derived using the sub-optimal algorithm mentioned in Section \ref{sec:application1}. We then add the constraints to the collection for upcoming queries.

We use Pandas as our execution engine by applying predicates to Pandas data frames. Similar to previous experiment, we evaluate the quality of the result and compare our predicate-constraint-based approach with AQP (20\% sampling) using two metrics: failure rate and distance to the true value.

The 100 group-by queries are decompose to 18500 predicate-only queries. And 3284 of the decomposed queries yields non-empty results. 

AQP using 20\% samples fails to bound 1964 of the queries, with a failure rate of 60\% (1964/3284).
Predicate-constraint approach generates bound for 59 queries and fails to derive bounds for the rest of the queries: the failure rate is 0 but coverage is only 2\%.

The average distance to the true bound for AQP is 14 and 260 for predicate-constraint-based approach.

As expected, above result indicates that even though AQP has a higher coverage it is not reliable. Predicate-constraint always generates true bounds but its performance depends on the constraints collected. We would expect the performance of predicate-constraint to increase as we collect more constraints. We could always provide a loose bound for 




==> reasoning-obselete.tex <==
\section{Extension to Complex Queries}
In this section, we use the basic framework described in the previous section and show how we can bound more complex queries.

\subsection{Reasoning Framework}
\label{sec:reasoning}
Our key insight is that we can consider the relational operators, filters and joins, as directly operating on the predicate-constraint sets that define the base relations.
We propagate the predicate-constraint sets to the top of the operator tree and then reduce it to the single relation problem described in the previous section. 

This can be thought of as defining a closed algebra over the predicate-constraint sets.
In our model, we assume that there are predicate-constraint sets defined for each base relation.
Our goal is to define how relational operators transform these sets.
We focus on two such operators $\sigma$ and $\times$ (joins can be handled as the combination of the two).

Suppose, we have two relations $R$ and $T$ and on these two relations there are two input predicate-constraint sets $\mathcal{S}_R$ and $\mathcal{S}_T$ respectively. We describe how each operator affects these sets:

\vspace{0.5em} \noindent \textbf{Select $R' = \sigma_p(R)$:} To handle selections, we simply apply the predicate to each of the predicate constraint elements. Define a dummy predicate constraint $\pi_p = (p,\mathcal{D},(0,\infty))$:
\[\mathcal{S}' = \{\pi \cdot \pi_p : \forall \pi \in \mathcal{S}_R \}\]

\vspace{0.5em} \noindent \textbf{Group By:} We handle group by aggregates by reduction to independent selections. We assume that we know the domain of the group by attributes in advance and bound the aggregate for each group independently.

\vspace{0.5em} \noindent \textbf{Cartesian $R' = R \times T$:} To handle the Cartesian operator, we use the direct-product operator:
\[\mathcal{S}' = \{\pi_i \times \pi_j : \forall \pi_i, \pi_j \in \mathcal{S}_R, \mathcal{S}_T \}\]

% \subsection{Optimality}

% \noindent\textbf{Select $R' = \sigma_p(R)$: } For a predicate-constraint $\mathcal{S}_R$ and another $\mathcal{S}_{R'}$ calculated by the approach given by Section~\ref{sec:reasoning}, we will prove that $\mathcal{D}=\mathcal{D}'$ where $\mathcal{D}=\{\sigma_p(R): R\models\mathcal{S}_R\}$ and $\mathcal{D}'=\{R':R'\models \mathcal{S}_{R'}\}$. This guarantees that for any function $f(\cdot)$ we have \[\max_{R\models\mathcal{S}_R} f(\sigma_p(R))=\max_{R'\models \mathcal{S}_{R'}} f(R')\] Intuitively, the right hand represents the optimal solution if we specify the constraints in the ``new'' form, and the left hand represents the optimal solution if we specify the constraints in the ``old'' form. \zs{we need the assumption that the lower bound for all attribute is 0 and the lower bound for cardinality is also 0.} \zs{I think I can fix this in another way. let me think about this.}

% For any $r\in\mathcal{D}$, consider one predicate-constraint $\pi=(\psi,\nu,\kappa)$ at a time. If $r\models\pi$, then $r\models\pi'=(\psi\cdot{}p,\nu,\kappa)$. And if $r\models\pi'$, $\sigma_p(r)\models\pi'$. Then we have $r\models\mathcal{S}_{R'}$, and  thus $r\in\mathcal{D}'$.

% For any $r\in\mathcal{D'}$, we have $r\models\mathcal{S}_R$: consider each $\pi\in\mathcal{S}_R$, $r\models\pi\cdot{}p$ gives $r\models\pi$. And it is clear that $\sigma_p(r)=r$. Thus we have $r\in\mathcal{D}$. This completes the proof that $\mathcal{D}=\mathcal{D'}$.

\zs{I guess proving the optimality does not make sense right now. We could still prove the above approach gives a bound. However, since we cannot compute the bound (due to the size of the final PCs), this proof seems to be not necessary. And the counterexample of this seems to be not necessary either.}



% \subsection{3-Way Join Counterexample}
% The bounds achieved by our framework are not tight from joins with more than 2 relations.
% The counter-example is the well-known worst-case optimal join result~\cite{ngo2018worst}. 
% This suboptimality arises because the reasoning framework handles joins in a pairwise way. If join condition links tables in a complex way, the reasoning framework may be overly conservative in the way it bounds the join. This point is important to restate. While the bounds are suboptimal for general n-way joins, they are loose (the bound is still correct, but there may not exist a valid relation that could have produced that bound).

% \begin{proposition}[Sub-Optimality of Bounds]
% For queries of more than 2 relations, the bounds can be exponentially loose in the number of relations.
% \end{proposition}
% \begin{proof}[Sketch]
% Consider the exemplary triangle counting query:
% \[q = |R(a,b)S(b,c)T(c,a)|\]
% Suppose, each relation has a size of $N$.
% Due to a fractional edge-cover bound, the maximum value of q is $O(N^{\frac{3}{2}})$~\cite{ngo2018worst}. If we apply our technique to bound $q$ for a predicate-constraint set defined for each relation, the bound would be $O(N^{3})$.
% We can perpetuate this logic to the 4-clique counting query, 5-clique, and so on:
% \[q = |R(a,b,c)S(b,c,d)T(c,d,e)U(e,a,b)|\], and the gap between the theoretical bound and the one computed by our framework grows exponentially.
% \end{proof}








==> shepherdcover.tex <==
\begin{center}
\textbf{Cover Letter}    
\end{center}

We thank the reviewers for their careful review of our revision and the conditional acceptance as a short paper. 

To fit in 10 pages, we reorganized the paper by moving Section 5 (an extension of our framework to joins) and the experiments following Section 6.3.1 to the appendix. We addressed every point in Section 12 of the reviews and our changes for shepherding are colored in blue. In the rest of this letter, we elaborate the changes we made. 

\vspace{.5cm}
\noindent{\textbf{Reviewer \#2}}

\Rev{R2.12.1}{
 I appreciate the detailed discussion on complexity in the response letter, but it is not completely clear to me. e.g., in Defn 0.2: if k <= 1, ie. there are " at most k (= 1) equality clauses on a single attribute (attribute equal to a constant)", then why should there be two PCs? And why should they completely overlap or be disjoint? In addition, I do not see any update in section 4.3 clarifying that combined complexity has been considered. 
}

\Ans{\todo{}}

\Rev{R2.12.1}{Understanding some details requires moving back and forth across sections, e.g., it is a critical assumption that the predicates can only be defined on individual input tables, and not on any joins of the tables or any aggregates, this is unclear and confusing when one reads section 2.}

\Ans{\todo{}}

\noindent{\textbf{Reviewer \#3}}

\Rev{R3.12.1}{
Still, the current version requires the reader spending time in interpreting what the authors could have meant, instead of the author having done that for the reader. A simple example is the sentence "Suppose, we are given a set of tables each with an unknown number of rows and a distribution of missing rows" It is not clear what distribution here really means. One could find out by jumping across different sections of the paper and reading between the lines, which makes it very unpleasant to read. 
}

\Ans{
\todo{Please revise.} Our framework does not make any assumption on the distribution of missing rows. In experiment \ref{sec:missing_ratio}, we investigate a typical scenarios where the distribution of the missing rows are correlated to PC. The other situation is when the distribution of missing rows is irrelevant to PC, in such case, PC can still generate a bound which is less accurate than the previous scenario. 
}

\Rev{R3.12.2}{
The new motivating example in 2.1 does not have joins, not even a group by. So the whole subtlety on correlations does not become clear. 
}
\Ans{GROUP-BY queries can be easily handled by our framework if we consider each GROUP-BY query as a combination of several simple queries without a GROUP-BY clause. We make this point clear in Section \ref{sec:background}. \todo{We further discuss joins in Section \ref{sec:joins} of the appendix}}

\Rev{R3.12.3}{
I found the basic definitions hard to follow, e.g. even the basic connection between predicates and frequency constraints. E.g. what does it now mean that a predicate has say (5, 10)? The predicate needs to appear at least 5 times? (I have to guess because the related paragraph does not define what the k’s mean).
}
\Ans{In Section \ref{sec:pc-exp}, we improved the definition of \textbf{Frequency Constraint} to explicitly define $k$. We also added some more details in the examples to explicitly refer to each component of a predicate constraint to make the basic definitions easier to understand.}

\Rev{R3.12.4}{
Should the paper be accepted as a short paper, I recommend the authors to move details or possibly all of the experiments (currently 6 pages) to the appendix yet not cut on the motivating examples and formal definitions.
}
\Ans{\todo{As discussed with the shepherd, we ... }}

==> teaser-1.tex <==
\begin{table}[t]
{\centering \sf SELECT AVG(age)
FROM Patient
GROUP BY pcp}

\vspace{0.5em}

\begin{tabular}{|l|llll|}
\hline
id & \multicolumn{1}{l|}{name} & \multicolumn{1}{l|}{pcp} & \multicolumn{1}{l|}{age} & \multicolumn{1}{l|}{zip} \\ \hline
1  & John Davis                & 0332-4                   & \textbf{?}                       & 60616                        \\ \cline{1-1}
2  & Janet Black               & 0110-0                   & 21                       & 60654                    \\ \cline{1-1}
3  & Tim Smith                 & 9961-3                   & \textbf{?}                       & 60250                     \\ \cline{1-1}
.. & ..                        & ..                       & ..                       & ..                       \\ \cline{1-1}
\hline

\end{tabular}
\vspace{0.5em}

\caption{A table of Hospital records with missing \texttt{age} values. We wish to find the average age of patients grouped by the \texttt{pcp} attribute. \label{teaser}}
\end{table}

==> teaser-2.tex <==
\begin{figure}

{\centering \sf SELECT AVG(age)
FROM Patient
GROUP BY pcp}

\vspace{0.75em}

{$c1: true \implies (0 <= age <= 122)$ }

{$freq(true) = |Patient|,$ }

\vspace{0.75em}

{$c2: \text{(pcp = 0332-4)} \implies (0 <= age <= 18)~~$ }

{$freq((pcp = 0332-4)) = |\sigma_{pcp = 0332-4}(Patient)|$ }

\vspace{0.75em}

{$c3: \text{(100 <= age <=122)} \implies (100 <= age <=122)~~$ }

{$freq((100 <= age <=122)) < 10$ }

\caption{Predicate-Constraint sets are sets of predicates that imply constraints on the values and frequency of missing data. (c1) Describes how all patients have an age less than 122, (c2) describes how all of the patients for a particular provider are under 18, and (c3) defines that there are no more than 10 patient above 100 years old. \label{teaser-2}}
\end{figure}
